Measurements of jet quenching with semi-inclusive hadron+jet distributions in Au+Au collisions at $\sqrt{s_{NN}}$ = 200 GeV

The STAR Collaboration reports the measurement of semi-inclusive distributions of charged-particle jets recoiling from a high transverse momentum hadron trigger, in central and peripheral Au+Au collisions at $\sqrt{s_{NN}}$ = 200 GeV. Charged jets are reconstructed with the anti-kT algorithm for jet radii R between 0.2 and 0.5 and with low infrared cutoff of track constituents ($p_T>0.2$ GeV/c). A novel mixed-event technique is used to correct the large uncorrelated background present in heavy ion collisions. Corrected recoil jet distributions are reported at mid-rapidity, for charged-jet transverse momentum $p_T^\mathrm{jet,ch}<30$ GeV/c. Comparison is made to similar measurements for Pb+Pb collisions at $\sqrt{s_{NN}}$ = 2.76 TeV, to calculations for p+p collisions at $\sqrt{s}$ = 200 GeV based on the PYTHIA Monte Carlo generator and on a Next-to-Leading Order perturbative QCD approach, and to theoretical calculations incorporating jet quenching. The recoil jet yield is suppressed in central relative to peripheral collisions, with the magnitude of the suppression corresponding to medium-induced charged energy transport out of the jet cone of $2.8\pm0.2\mathrm{(stat)}\pm1.5\mathrm{(sys)}$ GeV/c, for $10<p_T^\mathrm{jet,ch}<20$ GeV/c and R = 0.5. No medium-induced change in jet shape is observed for $R<0.5$. The azimuthal distribution of low-$p_T^\mathrm{jet,ch}$ recoil jets may be enhanced at large azimuthal angles to the trigger axis, due to scattering off quasi-particles in the hot QCD medium. Measurement of this distribution gives a 90% statistical confidence upper limit to the yield enhancement at large deflection angles in central Au+Au collisions of $50\pm30\mathrm{(sys)\%}$ of the large-angle yield in p+pcollisions predicted by PYTHIA.

==> Author.tex <==
\author{
L.~Adamczyk$^{1}$,
J.~K.~Adkins$^{19}$,
G.~Agakishiev$^{17}$,
M.~M.~Aggarwal$^{31}$,
Z.~Ahammed$^{50}$,
N.~N.~Ajitanand$^{40}$,
I.~Alekseev$^{15,26}$,
D.~M.~Anderson$^{42}$,
R.~Aoyama$^{46}$,
A.~Aparin$^{17}$,
D.~Arkhipkin$^{3}$,
E.~C.~Aschenauer$^{3}$,
M.~U.~Ashraf$^{45}$,
A.~Attri$^{31}$,
G.~S.~Averichev$^{17}$,
X.~Bai$^{7}$,
V.~Bairathi$^{27}$,
A.~Behera$^{40}$,
R.~Bellwied$^{44}$,
A.~Bhasin$^{16}$,
A.~K.~Bhati$^{31}$,
P.~Bhattarai$^{43}$,
J.~Bielcik$^{10}$,
J.~Bielcikova$^{11}$,
L.~C.~Bland$^{3}$,
I.~G.~Bordyuzhin$^{15}$,
J.~Bouchet$^{18}$,
J.~D.~Brandenburg$^{36}$,
A.~V.~Brandin$^{26}$,
D.~Brown$^{23}$,
I.~Bunzarov$^{17}$,
J.~Butterworth$^{36}$,
H.~Caines$^{54}$,
M.~Calder{\'o}n~de~la~Barca~S{\'a}nchez$^{5}$,
J.~M.~Campbell$^{29}$,
D.~Cebra$^{5}$,
I.~Chakaberia$^{3}$,
P.~Chaloupka$^{10}$,
Z.~Chang$^{42}$,
N.~Chankova-Bunzarova$^{17}$,
A.~Chatterjee$^{50}$,
S.~Chattopadhyay$^{50}$,
X.~Chen$^{37}$,
J.~H.~Chen$^{39}$,
X.~Chen$^{21}$,
J.~Cheng$^{45}$,
M.~Cherney$^{9}$,
W.~Christie$^{3}$,
G.~Contin$^{22}$,
H.~J.~Crawford$^{4}$,
S.~Das$^{7}$,
L.~C.~De~Silva$^{9}$,
R.~R.~Debbe$^{3}$,
T.~G.~Dedovich$^{17}$,
J.~Deng$^{38}$,
A.~A.~Derevschikov$^{33}$,
L.~Didenko$^{3}$,
C.~Dilks$^{32}$,
X.~Dong$^{22}$,
J.~L.~Drachenberg$^{20}$,
J.~E.~Draper$^{5}$,
L.~E.~Dunkelberger$^{6}$,
J.~C.~Dunlop$^{3}$,
L.~G.~Efimov$^{17}$,
N.~Elsey$^{52}$,
J.~Engelage$^{4}$,
G.~Eppley$^{36}$,
R.~Esha$^{6}$,
S.~Esumi$^{46}$,
O.~Evdokimov$^{8}$,
J.~Ewigleben$^{23}$,
O.~Eyser$^{3}$,
R.~Fatemi$^{19}$,
S.~Fazio$^{3}$,
P.~Federic$^{11}$,
P.~Federicova$^{10}$,
J.~Fedorisin$^{17}$,
Z.~Feng$^{7}$,
P.~Filip$^{17}$,
E.~Finch$^{47}$,
Y.~Fisyak$^{3}$,
C.~E.~Flores$^{5}$,
L.~Fulek$^{1}$,
C.~A.~Gagliardi$^{42}$,
D.~ Garand$^{34}$,
F.~Geurts$^{36}$,
A.~Gibson$^{49}$,
M.~Girard$^{51}$,
D.~Grosnick$^{49}$,
D.~S.~Gunarathne$^{41}$,
Y.~Guo$^{18}$,
A.~Gupta$^{16}$,
S.~Gupta$^{16}$,
W.~Guryn$^{3}$,
A.~I.~Hamad$^{18}$,
A.~Hamed$^{42}$,
A.~Harlenderova$^{10}$,
J.~W.~Harris$^{54}$,
L.~He$^{34}$,
S.~Heppelmann$^{32}$,
S.~Heppelmann$^{5}$,
A.~Hirsch$^{34}$,
G.~W.~Hoffmann$^{43}$,
S.~Horvat$^{54}$,
T.~Huang$^{28}$,
B.~Huang$^{8}$,
X.~ Huang$^{45}$,
H.~Z.~Huang$^{6}$,
T.~J.~Humanic$^{29}$,
P.~Huo$^{40}$,
G.~Igo$^{6}$,
P.~M.~Jacobs$^{22}$,
W.~W.~Jacobs$^{14}$,
A.~Jentsch$^{43}$,
J.~Jia$^{3,40}$,
K.~Jiang$^{37}$,
S.~Jowzaee$^{52}$,
E.~G.~Judd$^{4}$,
S.~Kabana$^{18}$,
D.~Kalinkin$^{14}$,
K.~Kang$^{45}$,
K.~Kauder$^{52}$,
H.~W.~Ke$^{3}$,
D.~Keane$^{18}$,
A.~Kechechyan$^{17}$,
Z.~Khan$^{8}$,
D.~P.~Kiko\l{}a~$^{51}$,
I.~Kisel$^{12}$,
A.~Kisiel$^{51}$,
L.~Kochenda$^{26}$,
M.~Kocmanek$^{11}$,
T.~Kollegger$^{12}$,
L.~K.~Kosarzewski$^{51}$,
A.~F.~Kraishan$^{41}$,
P.~Kravtsov$^{26}$,
K.~Krueger$^{2}$,
N.~Kulathunga$^{44}$,
L.~Kumar$^{31}$,
J.~Kvapil$^{10}$,
J.~H.~Kwasizur$^{14}$,
R.~Lacey$^{40}$,
J.~M.~Landgraf$^{3}$,
K.~D.~ Landry$^{6}$,
J.~Lauret$^{3}$,
A.~Lebedev$^{3}$,
R.~Lednicky$^{17}$,
J.~H.~Lee$^{3}$,
X.~Li$^{37}$,
C.~Li$^{37}$,
W.~Li$^{39}$,
Y.~Li$^{45}$,
J.~Lidrych$^{10}$,
T.~Lin$^{14}$,
M.~A.~Lisa$^{29}$,
H.~Liu$^{14}$,
P.~ Liu$^{40}$,
Y.~Liu$^{42}$,
F.~Liu$^{7}$,
T.~Ljubicic$^{3}$,
W.~J.~Llope$^{52}$,
M.~Lomnitz$^{22}$,
R.~S.~Longacre$^{3}$,
S.~Luo$^{8}$,
X.~Luo$^{7}$,
G.~L.~Ma$^{39}$,
L.~Ma$^{39}$,
Y.~G.~Ma$^{39}$,
R.~Ma$^{3}$,
N.~Magdy$^{40}$,
R.~Majka$^{54}$,
D.~Mallick$^{27}$,
S.~Margetis$^{18}$,
C.~Markert$^{43}$,
H.~S.~Matis$^{22}$,
K.~Meehan$^{5}$,
J.~C.~Mei$^{38}$,
Z.~ W.~Miller$^{8}$,
N.~G.~Minaev$^{33}$,
S.~Mioduszewski$^{42}$,
D.~Mishra$^{27}$,
S.~Mizuno$^{22}$,
B.~Mohanty$^{27}$,
M.~M.~Mondal$^{13}$,
D.~A.~Morozov$^{33}$,
M.~K.~Mustafa$^{22}$,
Md.~Nasim$^{6}$,
T.~K.~Nayak$^{50}$,
J.~M.~Nelson$^{4}$,
M.~Nie$^{39}$,
G.~Nigmatkulov$^{26}$,
T.~Niida$^{52}$,
L.~V.~Nogach$^{33}$,
T.~Nonaka$^{46}$,
S.~B.~Nurushev$^{33}$,
G.~Odyniec$^{22}$,
A.~Ogawa$^{3}$,
K.~Oh$^{35}$,
V.~A.~Okorokov$^{26}$,
D.~Olvitt~Jr.$^{41}$,
B.~S.~Page$^{3}$,
R.~Pak$^{3}$,
Y.~Pandit$^{8}$,
Y.~Panebratsev$^{17}$,
B.~Pawlik$^{30}$,
H.~Pei$^{7}$,
C.~Perkins$^{4}$,
P.~ Pile$^{3}$,
J.~Pluta$^{51}$,
K.~Poniatowska$^{51}$,
J.~Porter$^{22}$,
M.~Posik$^{41}$,
A.~M.~Poskanzer$^{22}$,
N.~K.~Pruthi$^{31}$,
M.~Przybycien$^{1}$,
J.~Putschke$^{52}$,
H.~Qiu$^{34}$,
A.~Quintero$^{41}$,
S.~Ramachandran$^{19}$,
R.~L.~Ray$^{43}$,
R.~Reed$^{23}$,
M.~J.~Rehbein$^{9}$,
H.~G.~Ritter$^{22}$,
J.~B.~Roberts$^{36}$,
O.~V.~Rogachevskiy$^{17}$,
J.~L.~Romero$^{5}$,
J.~D.~Roth$^{9}$,
L.~Ruan$^{3}$,
J.~Rusnak$^{11}$,
O.~Rusnakova$^{10}$,
N.~R.~Sahoo$^{42}$,
P.~K.~Sahu$^{13}$,
S.~Salur$^{22}$,
J.~Sandweiss$^{54}$,
M.~Saur$^{11}$,
J.~Schambach$^{43}$,
A.~M.~Schmah$^{22}$,
W.~B.~Schmidke$^{3}$,
N.~Schmitz$^{24}$,
B.~R.~Schweid$^{40}$,
J.~Seger$^{9}$,
M.~Sergeeva$^{6}$,
P.~Seyboth$^{24}$,
N.~Shah$^{39}$,
E.~Shahaliev$^{17}$,
P.~V.~Shanmuganathan$^{23}$,
M.~Shao$^{37}$,
A.~Sharma$^{16}$,
M.~K.~Sharma$^{16}$,
W.~Q.~Shen$^{39}$,
Z.~Shi$^{22}$,
S.~S.~Shi$^{7}$,
Q.~Y.~Shou$^{39}$,
E.~P.~Sichtermann$^{22}$,
R.~Sikora$^{1}$,
M.~Simko$^{11}$,
S.~Singha$^{18}$,
M.~J.~Skoby$^{14}$,
N.~Smirnov$^{54}$,
D.~Smirnov$^{3}$,
W.~Solyst$^{14}$,
L.~Song$^{44}$,
P.~Sorensen$^{3}$,
H.~M.~Spinka$^{2}$,
B.~Srivastava$^{34}$,
T.~D.~S.~Stanislaus$^{49}$,
M.~Strikhanov$^{26}$,
B.~Stringfellow$^{34}$,
T.~Sugiura$^{46}$,
M.~Sumbera$^{11}$,
B.~Summa$^{32}$,
Y.~Sun$^{37}$,
X.~M.~Sun$^{7}$,
X.~Sun$^{7}$,
B.~Surrow$^{41}$,
D.~N.~Svirida$^{15}$,
A.~H.~Tang$^{3}$,
Z.~Tang$^{37}$,
A.~Taranenko$^{26}$,
T.~Tarnowsky$^{25}$,
A.~Tawfik$^{53}$,
J.~Th{\"a}der$^{22}$,
J.~H.~Thomas$^{22}$,
A.~R.~Timmins$^{44}$,
D.~Tlusty$^{36}$,
T.~Todoroki$^{3}$,
M.~Tokarev$^{17}$,
S.~Trentalange$^{6}$,
R.~E.~Tribble$^{42}$,
P.~Tribedy$^{3}$,
S.~K.~Tripathy$^{13}$,
B.~A.~Trzeciak$^{10}$,
O.~D.~Tsai$^{6}$,
T.~Ullrich$^{3}$,
D.~G.~Underwood$^{2}$,
I.~Upsal$^{29}$,
G.~Van~Buren$^{3}$,
G.~van~Nieuwenhuizen$^{3}$,
A.~N.~Vasiliev$^{33}$,
F.~Videb{\ae}k$^{3}$,
S.~Vokal$^{17}$,
S.~A.~Voloshin$^{52}$,
A.~Vossen$^{14}$,
G.~Wang$^{6}$,
Y.~Wang$^{7}$,
F.~Wang$^{34}$,
Y.~Wang$^{45}$,
J.~C.~Webb$^{3}$,
G.~Webb$^{3}$,
L.~Wen$^{6}$,
G.~D.~Westfall$^{25}$,
H.~Wieman$^{22}$,
S.~W.~Wissink$^{14}$,
R.~Witt$^{48}$,
Y.~Wu$^{18}$,
Z.~G.~Xiao$^{45}$,
W.~Xie$^{34}$,
G.~Xie$^{37}$,
J.~Xu$^{7}$,
N.~Xu$^{22}$,
Q.~H.~Xu$^{38}$,
Y.~F.~Xu$^{39}$,
Z.~Xu$^{3}$,
Y.~Yang$^{28}$,
Q.~Yang$^{37}$,
C.~Yang$^{38}$,
S.~Yang$^{3}$,
Z.~Ye$^{8}$,
Z.~Ye$^{8}$,
L.~Yi$^{54}$,
K.~Yip$^{3}$,
I.~-K.~Yoo$^{35}$,
N.~Yu$^{7}$,
H.~Zbroszczyk$^{51}$,
W.~Zha$^{37}$,
Z.~Zhang$^{39}$,
X.~P.~Zhang$^{45}$,
J.~B.~Zhang$^{7}$,
S.~Zhang$^{37}$,
J.~Zhang$^{21}$,
Y.~Zhang$^{37}$,
J.~Zhang$^{22}$,
S.~Zhang$^{39}$,
J.~Zhao$^{34}$,
C.~Zhong$^{39}$,
L.~Zhou$^{37}$,
C.~Zhou$^{39}$,
X.~Zhu$^{45}$,
Z.~Zhu$^{38}$,
M.~Zyzak$^{12}$
}
\collaboration{STAR Collaboration}\noaffiliation
\address{$^{1}$AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\address{$^{2}$Argonne National Laboratory, Argonne, Illinois 60439}
\address{$^{3}$Brookhaven National Laboratory, Upton, New York 11973}
\address{$^{4}$University of California, Berkeley, California 94720}
\address{$^{5}$University of California, Davis, California 95616}
\address{$^{6}$University of California, Los Angeles, California 90095}
\address{$^{7}$Central China Normal University, Wuhan, Hubei 430079}
\address{$^{8}$University of Illinois at Chicago, Chicago, Illinois 60607}
\address{$^{9}$Creighton University, Omaha, Nebraska 68178}
\address{$^{10}$Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\address{$^{11}$Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\address{$^{12}$Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\address{$^{13}$Institute of Physics, Bhubaneswar 751005, India}
\address{$^{14}$Indiana University, Bloomington, Indiana 47408}
\address{$^{15}$Alikhanov Institute for Theoretical and Experimental Physics, Moscow 117218, Russia}
\address{$^{16}$University of Jammu, Jammu 180001, India}
\address{$^{17}$Joint Institute for Nuclear Research, Dubna, 141980, Russia}
\address{$^{18}$Kent State University, Kent, Ohio 44242}
\address{$^{19}$University of Kentucky, Lexington, Kentucky, 40506-0055}
\address{$^{20}$Lamar University, Physics Department, Beaumont, Texas 77710}
\address{$^{21}$Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000}
\address{$^{22}$Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\address{$^{23}$Lehigh University, Bethlehem, PA, 18015}
\address{$^{24}$Max-Planck-Institut fur Physik, Munich 80805, Germany}
\address{$^{25}$Michigan State University, East Lansing, Michigan 48824}
\address{$^{26}$National Research Nuclear University MEPhI, Moscow 115409, Russia}
\address{$^{27}$National Institute of Science Education and Research, Bhubaneswar 751005, India}
\address{$^{28}$National Cheng Kung University, Tainan 70101 }
\address{$^{29}$Ohio State University, Columbus, Ohio 43210}
\address{$^{30}$Institute of Nuclear Physics PAN, Cracow 31-342, Poland}
\address{$^{31}$Panjab University, Chandigarh 160014, India}
\address{$^{32}$Pennsylvania State University, University Park, Pennsylvania 16802}
\address{$^{33}$Institute of High Energy Physics, Protvino 142281, Russia}
\address{$^{34}$Purdue University, West Lafayette, Indiana 47907}
\address{$^{35}$Pusan National University, Pusan 46241, Korea}
\address{$^{36}$Rice University, Houston, Texas 77251}
\address{$^{37}$University of Science and Technology of China, Hefei, Anhui 230026}
\address{$^{38}$Shandong University, Jinan, Shandong 250100}
\address{$^{39}$Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\address{$^{40}$State University Of New York, Stony Brook, NY 11794}
\address{$^{41}$Temple University, Philadelphia, Pennsylvania 19122}
\address{$^{42}$Texas A\&M University, College Station, Texas 77843}
\address{$^{43}$University of Texas, Austin, Texas 78712}
\address{$^{44}$University of Houston, Houston, Texas 77204}
\address{$^{45}$Tsinghua University, Beijing 100084}
\address{$^{46}$University of Tsukuba, Tsukuba, Ibaraki, Japan,}
\address{$^{47}$Southern Connecticut State University, New Haven, CT, 06515}
\address{$^{48}$United States Naval Academy, Annapolis, Maryland, 21402}
\address{$^{49}$Valparaiso University, Valparaiso, Indiana 46383}
\address{$^{50}$Variable Energy Cyclotron Centre, Kolkata 700064, India}
\address{$^{51}$Warsaw University of Technology, Warsaw 00-661, Poland}
\address{$^{52}$Wayne State University, Detroit, Michigan 48201}
\address{$^{53}$World Laboratory for Cosmology and Particle Physics (WLCAPP), Cairo 11571, Egypt}
\address{$^{54}$Yale University, New Haven, Connecticut 06520}
